Communication-Efficient Secure Aggregation in Decentralized Learning

Decentralized learning (DL) enables participants to collaboratively train models without a central server, yet it faces significant scalability challenges that demand sparsification to reduce the prohibitive communication costs of peer-to-peer exchange. While secure aggregation effectively mitigates privacy risks in standard settings, it has remained fundamentally incompatible with sparsification in decentralized networks due to the mismatch of indices across local updates, forcing a trade-off between communication efficiency and privacy. This paper introduces CESAR, a novel protocol that resolves this incompatibility by integrating secure aggregation and sparsification to provide provable defense against honest-but-curious and colluding adversaries. By coordinating masks over parameter intersections, CESAR supports node dropouts and robust privacy without central aggregation. Empirical evaluations on models up to 124 million parameters demonstrate that CESAR matches the accuracy of non-private baselines while cutting total data exchange by 66.7 % compared to a standard full-parameter decentralized protocol (D-PSGD). With TopK sparsification on IID data, CESAR even exceeds by 0.3 % the accuracy achieved by D-PSGD with sparsification. Collectively, these results establish CESAR as the first decentralized protocol to achieve both privacy and communication efficiency through secure aggregation in DL.

==> tables/scalability_degree_table.tex <==
\pgfplotstableset{
   create on use/overhead_per_2_neighbours/.style={
   create col/expr={\thisrow{total_protocol_overhead_mean} / \thisrow{second_degree_neighbors}}}
}

\pgfplotstabletypeset[
   col sep=comma,
   columns={degree,total_protocol_overhead_mean,second_degree_neighbors,overhead_per_2_neighbours}, % Specify the columns to include
   columns/degree/.style={column name=\textbf{Degree}, column type={c}},
   columns/second_degree_neighbors/.style={
   		%column name=\begin{tabular}{@{}c@{}}\textbf{Average}\\\textbf{second-degree}\\\textbf{neighborhood}\\\textbf{size}\end{tabular}, column type={|c},
   		column name={\textbf{Avg. $2^{nd}$ deg. neighborhood size}}, column type={|C{20mm}},
   		precision=2},
   columns/total_protocol_overhead_mean/.style={
       %column name=\begin{tabular}{@{}c@{}}\textbf{\sys}\\\textbf{overhead}\\\textbf{[\si{GB}]}\end{tabular}, column type={|c},
       column name={\textbf{Overhead [\si{GB}]}}, column type={|C{14mm}},
       fixed, fixed zerofill, precision=2},
   columns/overhead_per_2_neighbours/.style={
       %column name=\begin{tabular}{@{}c@{}}\textbf{\sys}\\\textbf{overhead per}\\\textbf{second-degree}\\\textbf{neighbor [\si{GB}]}\end{tabular}, column type={|c},
       column name={\textbf{Overhead per $2^{nd}$ deg. neighbor [\si{GB}]}}, column type={|C{23mm}},
       fixed, fixed zerofill, precision=4},
   every head row/.style={before row=\toprule, after row=\midrule},
   %every nth row={1}{before row=\midrule},
   every last row/.style={after row=\bottomrule},
]{data/CIFAR/degree_scalability/cummulative_avg_data.csv}


==> tables/scalability_nodes_count_table.tex <==
\pgfplotstableset{
    create on use/param_data/.style={
    create col/expr={\thisrow{total_bytes_mean} + \thisrow{total_meta_mean}}}
}

\pgfplotstabletypeset[
    col sep=comma,
    columns={number_of_nodes, param_data, total_protocol_overhead_mean}, % Specify the columns to include
    columns/number_of_nodes/.style={column name=\textbf{Number of nodes}, column type={{C{20mm}}}},
    columns/param_data/.style={
        column name=\begin{tabular}{@{}c@{}}\textbf{Parameter data}\\\textbf{[\si{GB}]}\end{tabular}, column type={|c},
        precision=2},
    columns/total_protocol_overhead_mean/.style={
        column name=\begin{tabular}{@{}c@{}}\textbf{CESAR overhead}\\\textbf{[\si{GB}]}\end{tabular}, column type={|c},
        precision=2},
    every head row/.style={before row=\toprule, after row=\midrule},
    %every nth row={1}{before row=\midrule},
    every last row/.style={after row=\bottomrule},
]{data/CIFAR/scalability/cummulative_avg_data.csv}
